It is Time for New Perspectives on How to Fight Bloat in GP

The present and future of evolutionary algorithms depends on the proper use of modern parallel and distributed computing infrastructures. Although still sequential approaches dominate the landscape, available multi-core, many-core and distributed systems will make users and researchers to more frequently deploy parallel version of the algorithms. In such a scenario, new possibilities arise regarding the time saved when parallel evaluation of individuals are performed. And this time saving is particularly relevant in Genetic Programming. This paper studies how evaluation time influences not only time to solution in parallel/distributed systems, but may also affect size evolution of individuals in the population, and eventually will reduce the bloat phenomenon GP features. This paper considers time and space as two sides of a single coin when devising a more natural method for fighting bloat. This new perspective allows us to understand that new methods for bloat control can be derived, and the first of such a method is described and tested. Experimental data confirms the strength of the approach: using computing time as a measure of individuals' complexity allows to control the growth in size of genetic programming individuals.

==> backup-templates/templates/referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...´': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> parts_workshop/old/GPGPU.tex <==
Graphic Processing Units became to be used as high performance computation tools for general purpose at the first years of the XXI century. Then, around 2006 we find the first implementations of evolutionary algorithms on GPUs \cite{}\cite{}. Fitness Evaluation, as the most costly task, in terms of compuation effort, was the main objective of the first implementations of GP on GPUs made by Harding, Banzhaf and Langdom.

In \cite{harding2007fast} and \cite{harding2007fastb} authors show the use of the GPU as an evaluatir for GP expressions. They proposed to parse the trees which represent the GP expression only once, and parallelize the evaluation for all the test cases. The main process run in the GPU and the evaluations are computed on the GPU. At this time CUDA was only a promising project and the implemetation of the parser was made in c\#. The textures were prepared in the CPU and sent to shader processors, a converted into an array again to be evaluated. They applied their implementaion to basic becnhmarks and then to a classification problem in bioinformatics. Authour pointed out on of the main problems for EA on the GPU, the random number generation. In order to obtain quality random numbers the use an interesting cellular automata.


\subsection*{Fast Genetic Programming and Artificial Developmental Systems on GPUs}
In this paper we demonstrate the use of the Graphics
Processing Unit (GPU) to accelerate Evolutionary Computation
applications, in particular Genetic Programming approaches.
We show that it is possible to get speed increases
of several hundred times over a typical CPU implementation,
catapulting GPU processing for these applications
into the realm of HPC. This increase in performance also
extends to artificial developmental systems, where evolved
programs are used to construct cellular systems. Feasibility
of this approach to efficiently evaluate artificial developmental
systems based on cellular automata is demonstrated..\cite{harding2007fastb}
\subsection*{Graphics processing units and genetic programming: an overview}
A top end graphics card (GPU) plus a suitable
SIMD interpreter can deliver a several hundred fold speed
up, yet cost less than the computer holding it. We give
highlights of AI and computational intelligence applications
in the new field of general purpose computing on
graphics hardware (GPGPU). In particular, we surveyed
genetic programming (GP) use with GPU. We gave several
applications from Bioinformatics and showed that how the
fastest GP is based on an interpreter rather than compilation.
Finally using GP to generate GPU CUDA kernel
C?? code is sketched.\cite{langdon2011graphics}
\subsection*{Genetically improved CUDA C++ software}
%Resaltar que aquí cerramos el círculo
Genetic Programming (GP) may dramatically increase the performance of software written by domain experts. GP and autotuning are used to optimise and refactor legacy GPGPU C code for modern parallel graphics hardware and software. Speed ups of more than six times on recent nVidia GPU cards are reported compared to the original kernel on the same hardware.\cite{langdon2014genetically}
\subsection*{Nature-Inspired Meta-Heuristics on Modern GPUs:
State of the Art and Brief Survey of Selected Algorithms}
Graphic processing units (GPUs) emerged recently as an exciting new hardware
environment for a truly parallel implementation and execution of Nature and
Bio-inspired Algorithms with excellent price-to-power ratio. In contrast to common
multicore CPUs that contain up to tens of independent cores, the GPUs represent a
massively parallel single-instruction multiple-data devices that can nowadays reach
peak performance of hundreds and thousands of giga floating-point operations per second.
Nature and Bio-inspired Algorithms implement parallel optimization strategies in
which a single candidate solution, a group of candidate solutions (population), or multiple
populations seek for optimal solution or set of solutions of given problem. Genetic
algorithms (GA) constitute a family of traditional and very well-known nature-inspired
populational meta-heuristic algorithms that have proved its usefulness on a plethora of
tasks through the years. Differential evolution (DE) is another efficient populational
meta-heuristic algorithm for real-parameter optimization. Particle swarm optimization
(PSO) can be seen as nature-inspired multiagent method in which the interaction of
simple independent agents yields intelligent collective behavior. Simulated annealing
(SA) is global optimization algorithm which combines statistical mechanics and combinatorial
optimization with inspiration in metallurgy. This survey provides a brief
overview of the latest state-of-the-art research on the design, implementation, and
applications of parallel GA, DE, PSO, and SA-based methods on the GPUs.\cite{kromer2014nature}
\subsection*{A Genetic Programming Approach to Designing Convolutional
Neural Network Architectures}
%novedad y apliación
The convolutional neural network (CNN), which is one of the deep
learning models, has seen much success in a variety of computer
vision tasks. However, designing CNN architectures still requires
expert knowledge and a lot of trial and error. In this paper, we
attempt to automatically construct CNN architectures for an image
classification task based on Cartesian genetic programming (CGP).
In our method, we adopt highly functional modules, such as convolutional
blocks and tensor concatenation, as the node functions
in CGP. The CNN structure and connectivity represented by the
CGP encoding method are optimized to maximize the validation
accuracy. To evaluate the proposed method, we constructed a CNN
architecture for the image classification task with the CIFAR-10
dataset. The experimental result shows that the proposed method
can be used to automatically find the competitive CNN architecture
compared with state-of-the-art models.\cite{suganuma2017genetic}
\subsection*{Multi-objective genetic programming for feature
extraction and data visualization}
Feature extraction transforms high-dimensional data into a new subspace of lower dimensionality while keeping the classification accuracy. Traditional algorithms do not consider the multi-objective nature of this task. Data transformations should improve the classification performance on the new subspace, as well as to facilitate data visualization, which has attracted increasing attention in recent years. Moreover, new challenges arising in data mining, such as the need to deal with imbalanced data sets call for new algorithms capable of handling this type of data. This paper presents a Pareto-based multi-objective genetic programming algorithm for feature extraction and data visualization. The algorithm is designed to obtain data transformations that optimize the classification and visualization performance both on balanced and imbalanced data. Six classification and visualization measures are identified as objectives to be optimized by the multi-objective algorithm. The algorithm is evaluated and compared to 11 well-known feature extraction methods, and to the performance on the original high-dimensional data. Experimental results on 22 balanced and 20 imbalanced data sets show that it performs very well on both types of data, which is its significant advantage over existing feature extraction algorithms.
\cite{cano2017multi}
\subsection*{}
\subsection*{}
\subsection*{}


==> parts_workshop/old/ParallelGE.tex <==
Grammars are an essential tool in many aspects of computing. By means of a grammar we can represent in a formal and structured way a set of rules, which allows to transfer it easily to an algorithmic procedure. Since the beginnings of genetic programming, several approaches have been studied that specify how to generate solutions through grammars. This allows not only to improve the description but also to include knowledge in the search process. \cite{hidalgo2017embedded,mckay2010grammar,chennupati2014multi,pospichal2011acceleration,colmenar2016compilable,van2012automatic,chennupati2014efficiency}

\subsection{CPU}

\subsection*{On the efficiency of Multi-core Grammatical Evolution (MCGE) evolving multi-core parallel programs }
"In this paper we investigate a novel technique that optimizes the execution time of Grammatical Evolution through the usage of on-chip multiple processors. This technique, Multicore Grammatical Evolution (MCGE) evolves natively parallel programs with the help of OpenMP primitives through the grammars, such that not only can we exploit parallelism while evolving individuals, but the final individuals produced can also be executed on parallel architectures even outside the evolutionary system. We test MCGE on two difficult benchmark GP problems and show its efficiency in exploiting the power of the multicore architectures. We further discuss that, on these problems, the system evolves longer individuals while they are evaluated quicker than their serial implementation."
\subsection*{Multi-core GE: automatic evolution of CPU based multi-core parallel programs}
We describe the utilization of on-chip multiple CPU architectures
to automatically evolve parallel computer programs.
These programs have the capability of exploiting the
computational efficiency of the modern multi-core machines.
This is significantly different from other parallel EC approaches
because not only do we produce individuals that,
in their final form, can exploit parallel architectures, we can
also exploit the same parallel architecture during evolution
to reduce evolution time.
We use Grammatical Evolution along with OpenMP specific
grammars to produce natively parallel code, and demonstrate
that not only do we enjoy the benefit of final individuals
that can run in parallel, but that our system scales
effectively with the number of cores.



\subsection*{Automatic Discovery of Algorithms
for Multi-Agent Systems}
Automatic algorithm generation for large-scale distributed
systems is one of the holy grails of artificial intelligence and
agent-based modeling. It has direct applicability in future
engineered (embedded) systems, such as mesh networks of
sensors and actuators where there is a high need to harness
their capabilities via algorithms that have good scalability
characteristics.
NetLogo has been extensively used as a teaching and research
tool by computer scientists, for example for exploring
distributed algorithms. Inventing such an algorithm usually
involves a tedious reasoning process for each individual idea.
In this paper, we report preliminary results in our effort to
push the boundary of the discovery process even further, by
replacing the classical approach with a guided search strategy
that makes use of genetic programming targeting the
NetLogo simulator. The effort moves from a manual model
implementation to an automated discovery process. The
only activity that is required is the implementation of primitives
and the configuration of the tool-chain. In this paper,
we explore the capabilities of our framework by re-inventing
five well-known distributed algorithms.

\subsection{GPU}
Due to the decoding process through a grammar, parallelization is not an easy task for all platforms. For example, when parallelizing on a graphics card, if a good allocation of resources is not made, it is very difficult to achieve an efficient implementation. Therefore, to date there have been few parallel implementations of GE on GPUs. 
The necessity of using a grammar makes the efficient parallelization of  GE a difficult task. The are few works in the literature, \cite{Pospichal2011}, and they only presented results on symbolic regression problems. There are several problems which make the parallelization of GE programs a difficult process. \cite{Pospichal2011} and \cite{Hidalgo2017} propose two different implementations of GE on GPU. In the second one an specific implementation is performed for each grammar, taking advantage of the large number of multiprocessors of the GPU with the cost of reducing the versatility.

\subsection*{Compilable Phenotypes: Speeding-Up the Evaluation of Glucose Models in Grammatical Evolution}
This paper presents a method for accelerating the evaluation of individuals in Grammatical Evolution. The method is applied for identification and modeling problems, where, in order to obtain the fitness value of one individual, we need to compute a mathematical expression for different time events. We propose to evaluate all necessary values of each individual using only one mathematical Java code. For this purpose we take profit of the flexibility of grammars, which allows us to generate Java compilable expressions. We test the methodology with a real problem: modeling glucose level on diabetic patients. Experiments confirms that our approach (compilable phenotypes) can get up to 300x reductions in execution time.
\subsection*{Acceleration of grammatical evolution using graphics processing units: computational intelligence on consumer games and graphics hardware}
Several papers show that symbolic regression is suitable for data analysis and prediction in financial markets. Grammatical Evolution (GE), a grammar-based form of Genetic Programming (GP), has been successfully applied in solving various tasks including symbolic regression. However, often the computational effort to calculate the fitness of a solution in GP can limit the area of possible application and/or the extent of experimentation undertaken. This paper deals with utilizing mainstream graphics processing units (GPU) for acceleration of GE solving symbolic regression. GPU optimization details are discussed and the NVCC compiler is analyzed. We design an effective mapping of the algorithm to the CUDA framework, and in so doing must tackle constraints of the GPU approach, such as the PCI-express bottleneck and main memory transactions.

This is the first occasion GE has been adapted for running on a GPU. We measure our implementation running on one core of CPU Core i7 and GPU GTX 480 together with a GE library written in JAVA, GEVA.

Results indicate that our algorithm offers the same convergence, and it is suitable for a larger number of regression points where GPU is able to reach speedups of up to 39 times faster when compared to GEVA on a serial CPU code written in C. In conclusion, properly utilized, GPU can offer an interesting performance boost for GE tackling symbolic regression.

\subsection*{Embedded Grammars for Grammatical Evolution on GPGPU}
This paper presents an implementation of Grammatical Evolution on a GPU architecture. Our proposal, Embedded Grammars, implements the grammar directly in the code. Although more rigid, it allows to compute the decodification in parallel with the evaluation of the individuals. We tested three different grammars with a set of eight symbolic regression problems. The symbolic regression problems consists on obtaining a mathematical expression in the form   y=f(x) , in our case, from a set of 288 pairs x, y. The analysis of the results shows that Embedded Grammars are better not only in terms of execution time, but also in quality when compared with an implementation on a CPU. Speed-up results are also better than those presented in the literature.

\subsection{GP for classification}
Abstract—Classification is one of the most researched questions
in machine learning and data mining. A wide range of real problems
have been stated as classification problems, for example credit
scoring, bankruptcy prediction, medical diagnosis, pattern recognition,
text categorization, software quality assessment, and many
more.The use of evolutionary algorithms for training classifiers has
been studied in the past few decades. Genetic programming (GP) is
a flexible and powerful evolutionary technique with some features
that can be very valuable and suitable for the evolution of classifiers.
This paper surveys existing literature about the application of
genetic programming to classification, to show the different ways
in which this evolutionary algorithm can help in the construction
of accurate and reliable classifiers.
The main problem of GP is its computational cost, primarily
due to the computation of the fitness of individuals, which
has to be repeatedly evaluated through the evolutionary process.
Fitness evaluation is particularly costly when evolving classifiers,
since it implies the application of the classifier encoded
by each individual in the population to all the data instances
in the training set. Training times on the order of seconds [79],
[121], [122], [130], [134], minutes [51], [78], [80], [125], [137],
hours [68], [85], [153], or even days [63], [123] have been reported
in the literature reviewed in this paper.Parallel and distributed implementations
are probably the most obvious approach to decrease training
time, and are applied in [63], [73], [90], [109], [158], [168],
[171], [174], and [176].

==> parts_workshop/old/balancing.tex <==
The key idea is to distribute individuals to be evaluated among available processors.  Therefore, a load-balancing mechanism must be applied.  %The thing is that using such a mechanism has provided interesting new features that we describe below.

Load-balancing, as well as scheduling, are of paramount importance in the area of parallel and distributed computing.  The goal is to distribute task among processors as evenly as possible, reducing makespan.  Several possibilities are available, that may relay in static or dynamic load-balancing  (See \cite{Osman} \cite{Zaki}).  

GP presents interesting differences with more traditional EAs:  instead of using chromosomes with a previously established size, it relies on variable-size chromosomes, and this greatly affects the kind of load-balancing approach to be used.  A number of researchers have considered the implications of load-balancing in combination with parallel EAs (check for instance \cite{Zomaya}), but regarding GP, the implications of load-balancing approaches have been considered since the end of the ninetis.

Thus, Oussaidene et al in 1998 \cite{oussaidene1996parallel} described an embarrasingly parallel version of GP that considers complexity of individuals as the basis for establishing the load-balancing policy. Although those authors were aware of the importance of load-balancing techniques, they did not notice the relationship that may exist with the evolution of individuals' size, which is a well-known feature of GP.

Few papers since then have studied the importance of load-balancing techniques in GP. We may refer to \cite{preliminaryloadbalancing}, where several methods were tested. But again, no specific study on their relationship with the bloat phenomenon was presented. In any case, some of the main features that are involved in load-balancing approaches for GP are described below.  We may thus see that the area is still awaiting for improvements.



==> parts_workshop/old/beginnings.tex <==
The above referred models have been adopted by researchers progressively through history, when the problems addressed have been progressively harder, and thus the required longer time to be solved, and also hardware technology had developed offering what was required by each of the models.

As described in \cite{parallelgp}, few years after the publication of the influential book by Koza \cite{koza1990genetic}, the first parallel gp implementation was carried out by Tuffs \cite{tufts1993parallel}, which employed an embarrasingly parallel model.  Later on, Julli\`e and Pollack presented a fine-grained SIMD architecture, which included both parallelizaton of fitness cases, but also an island model employing a Ring topology.

Koza and Andre \cite{andre1996parallel} also described a parallel implementation of GP based on the Island Model, but using a network of transputers this time as the underlying hardware -single VLSI devices containing 32-bit on-chip processor, on-chip memory, and independent serial bi-direction physical on-chip communication links.  A client/server modelo using a central supervisory process and 64 transputers, each running an island.  A cellular topology was established for the connection among islands, so that every island communicated with 4 neighboring ones.  The main conclusion was that parallel gp delivered more that linear speedup, result that was questioned later by Punch in \cite{punch1998effective}.  His conclusion was that the problem selected, particularly the number of solutions availabe in the searche space, influences the performance of the Island Model:  multiple-solution problems would be more amenable to multiple populations than single-solution problems.

The first in-depth study on specific parameters of the Island Model was presented in 2000: firstly, Tongchim and Chongstitvatna studied syncronous and asynchronous models in \cite{tongchim2000nearest}, and then migration policies, topologies and deme sizes were studied in \cite{fernandez2003empirical}.  Similarly, the cellular model was studied in \cite{folino2003scalable}.

Since then, parallel GP models have been frequently adopted by researchers, and applied to many different hard optimization problems.  We described below the main features of each of the models....

==> parts_workshop/old/hidden_features.tex <==
%New parameters and properties.
\subsection{Bloat dynamics in the island model}

The \textit{bloat} phenomenon is a well known anomaly that is present in variable-size chromosome based evolutionary techniques, which is the case of GP.  As described in \cite{} number of reasons affects size evolutions of candidate solutions, which is a problem for GP, given that the longer the run, the larger the memory required for storing the population and the time required to evaluate individuals.

This phenomenon has been addressed frequently in the GP literature, and many proposals and reviews of the topics has already been published.  But also some interesting findings are associated with some of the parallel models previously described in the context of this problem.

Although spatially structured models were conceived as a method for improving the search capability of EAs, when it was applied to GP, not only this was achieved and diversity improved.  Moreover, a experimental analysis discovered first that Island model positively affected how the \textit{bloating} phenomenon occurred.

...

\subsection{Shrinking populations and Fault tolerance}

Traditionally, the number of individuals included in a population are stable from beginning to end.  Although this is the standard approach, nothing avoid to change the population size while an experiment is still running.

In 2002, a couple of papers described for the first time GP runs where decreasing population sizes were employed.  Actually, the first paper applying such an approach considered the relationship between the bloat phenomenon and the global size of the population regarding memory consumption \cite{}.  The idea thus was born in the sequential version of the GP algorithm, but again a connection between \textit{shrinking} populations and the well knwon \textit{churn} phenomenon that usually affect volunteer computing based models were discovered.

...

\subsection{Time and space considerations}


\subsection{Self and Ephemeral properties}



==> parts_workshop/old/intro_old.tex <==
Genetic Programming became popular from the mid-nineties onward, after \cite{koza1992} published his first book on the topic.  This machine learning technique has widely demonstrated capabilities for addressing difficult real-world problems, but a challenge remains:  the bloat phenomenon, see \cite{bloat}.

\subsection{Problem Statement}

According to \cite{fitnessandbloat} fitness improvement  clearly correlates with the inherent bloating behavior present in any evolutionary approach using variable-size chromosomes. Although many authors have addressed this problem from different perspectives, no perfect solution has yet been found, and there is still room for improvement.

This paper aims to provide new perspectives for fighting bloat, which may in the future allow development of a series of new bloat control methods based on function (chromosome) evaluation time.  Although there is a correlation between an individual's size and its evaluation time, the latter also depends on the underlying hardware infrastructure that is used to carry out the evaluation.  Therefore, the connection with parallel and distributed model architectures must be addressed.  Although island models have  been analyzed before in this context (\cite{fernandez1}, \cite{whigham}), these previous approaches relied more on spatial structure of the models, while we are here more interested in the standard GP algorithm, whether it is run sequentially or in parallel.  
%We then try to understand their basic behavior when modern parallel architectures are employed to run it, such as multicore based computer systems.  

By analyzing the intrinsic behavior of the algorithm, we show the space-time connection with the bloat phenomenon.  In addition, we show how this new relationship could benefit chromosome based EAs of variable size, enabling the development a new kind of bloat-control mechanisms that can naturally benefit from the underlying parallel processors that nowadays are present in every computer system, from handheld devices, desktop systems and large computer systems.

Therefore, we devise new ways of naturally controlling the bloat problem:  we analyze the bloat phenomenon using \textit{time} (execution time) instead of \textit{space} (memory consumption), although both are measures of a single entity: the time-space behavior of individuals.  We resort to the space-time continuum as a metaphor providing a new source of inspiration, and thus try to provide a new way for analyzing and fighting bloat.  To the best of our knowledge, this is the first time such an approach is described and applied, and the results we show demonstrate the usefulness of the idea, both in sequential and embarrassingly parallel versions of the algorithm, which opens new possibilities up in other parallel and distributed versions of GP.

\subsection{Research Contributions}

Thus, our main contribution here are (1) to properly establish a relationship between an individual's size and evaluation time, showing the advantages of using evaluation time when analyzing individuals' complexity.  Moreover, (2) we use such an approach to show that a new kind of bloat control mechanisms can be more naturally developed, and (3) we present the first such method based on fitness evaluation time, tested in both sequential and parallel executions of the algorithm.  Although many possibilities may be derived from the new perspective presented, this first method shows the usefulness of the approach, paving the way towards a new class of bloat control mechanisms.

%when the dynamics of parallel and distributed systems is taken into account, without any other consideration, such as spatial structures of the model.  The experiments performed, both by first considering the model, and then on a parallel infrastructure, show the interest of this proposal.

The rest of the paper is organized as follows:  In Section \ref{Complexity} we describe some GP-associated considerations that gave rise to the ideas developed later.  Section \ref{Bloat} reviews previous approaches for fighting bloat, and the main features of parallel models that may be taken into account when analyzing this problem. Then, Section \ref{Load} describes how load-balancing techniques could be of interest in this context. Section \ref{Methods} presents our proposal, while Section \ref{Results} shows the experiments performed and results obtained.  Finally, we draw our conclusions in Section \ref{Conclusions}.

==> parts_workshop/old/models.tex <==
%New parameters and properties.

By the age when Evolutionary Algorithms were first described, parallel and distributed systems were not easily accesible.  Yet, ideas about parallelization were present at that time \cite{fogel1998evolutionary}.  Thus, when GP drew attention in the mid-nineties, parallel architectures were more accesible, and that is why even in the early years of GP the models already described for EAs could be applied to GP. 

Nevertheless, as hardware technologies have improved, new distributed models have been developed, allowing to be also used by GP researchers to both run experiments faster and also get what every model offers for better solutions.

We describe here some of the main known models and features, and we will see later on some unexpected phenomena that has been reported in the last few years and helps to improve in the quality of results the models provide.

\subsection{Flynn and EAs}

%TO BE COMPLETED:  The idea is to show the taxonomy and relate it with the models described below.
During the last 20 years the growth in processor performance has been slowed down, though being important. From 1986 to 2002 aproximately performance increases about a 50\% per year, and from this year the increase reduced to 25 \% to 2011, 12 \% till 2015 and nowadays we are in a 3.5 \% of improvement per year. With the decline in performance improvement of processors, new forms of parallelism in applications have been developed. These come, on many occasions, from parallel techniques that already existed twenty years ago. With the technological improvement, some architectures and paradigms of programming abandoned by their difficulty of manufacture or implementation have returned to be reused today.

At present we can distinguish five main types of computers; Personal Mobile Devices, Embedded Computers, Servers and Clusters,  Warehouse Computers, and Destok Computers. Although there are parallel implementations of evolutionary algorithms in almost all the five categories, what is more usual is to see genetic programming being parallelized in the last 3 categories.


There are two levels of Parallelism to exploit

\begin{itemize}
\item Data level 
\item Thread level
\end{itemize}

There are four ways of exploiting those two levels of parallelism

\begin{itemize}
\item Instruction level
\item Vector architectures
\item Thread-level
\item Request level
\end{itemize}

Classsification of Parallel Computers by Flynn(1966)

\begin{itemize}
\item SISD
\item SIMD
\item MIMD
\item MISD
\end{itemize}


\subsection{Embarrassingly parallel models}
As described above, embarrassingly parallel models were the first choice for GP researchers when trying to make profit of several processors when running GP \cite{cantu2000efficient}. This easiest parallel model allows to evaluate fitness functions of several individuals simultaneously, sending different individuals to different processors in the evaluation step.  When the fitness function takes long, this is a nice improvement given that the main GP algorithm does not change:  every step is performed as always, and the master-client model is in charge of distributing and evaluating fitness cases when required.  And this is probably the reason why this model has been successfully applied with different hardware platforms: networks of transputers \cite{koza1995parallel}, clusters and grids \cite{lim2007efficient}, and more recently on GPUs \cite{wong2005parallel} and clouds \cite{garcia2015evospace}, and has been the most frequently used model;  researchers find it easy to parallelize just the fitness evaluation step, while the remaining parts of their code remains unchanged.  As we will see below, similarly as in other areas of software industry, the main reason for a parallel or distributed GP model to be applied is how easily it can be introduced in an already available sequential code.

This is the only model that does not change the main steps of the standard GP algorithm. But the parallel evaluation of individuals in different processors introduces some dynamics that must be consider for a proper implementation.  Particularly, load balancing methods should be considered in this context.

\subsubsection{Load Balancing}
\label{balancing}
\input{./parts/balancing.tex}


\subsection{The Island Model}

Despite the success of the master-client model described above, researchers were always aware of the Amdhal's law, which predict the gaining when parallelizing sequential code:  it depends on the portion of the sequential code being parallelized.  The longer the time this portion takes when solving the task, the larger the gainings \cite{gustafson1988reevaluating}.  Thus researchers soon decided to parallelize not just the fitness evaluation step, but also other more hidden parts of the algorithm which in the end implied a deep change in the dynamics of the underlying evolutionary process, opening new and previously unseen opportunities for improvements.

The \textit{island model} was soon devised as the next step to be performed:  researchers decided to split the main population of candidate solutions into several subpopulations -demes- so that a somehow independent evolutionary process could be run in different processors using each of the subpopulations \cite{tomassini2006spatially}.  Nevertheless, extra ingredients were required to avoid the undesired isolated model, with several algorithms simply running independently.  Although probably useful when several runs have to be launched, the model can scarcely be named as parallel, given that no connection exist among the processors.  Instead, a new \textit{migration} step was added, so that selected individuals could travel with a given frequency among islands.  Thus, every subpopulation run the standard algorithm, and from time to time, some individuals are exchanged among subpopulations with a given frequency.

The new model requires a number of extra parameters to be defined:  island size, frequency of migration, number of migrating
individuals, selection operator in charge of selecting migrants, discharging policy allowing to maintain the size of islands once new individuals arrive, etc.  Opportunities arose to study the influence of these set of parameters in the GP island based model \cite{fernandez2003empirical}.  Not only in GP but also in GA the studies showed the benefit of the migration process, which helps to promote diversity within subpopulations, and in the end, to more easily find solutions to the problems faced.  Therefore a double benefit came with the model:  parallelism on the one hand, which saves computing time, and diversity improvement, which also helps to find solutions quicker.

\subsection{The Cellular Model}

The island model is a well-known \textit{structured} model, although not the only one.  Structured models introduces a kind of structure within the population, and this helps diversity \cite{tomassini2006spatially}.  Not only the structure can be established by means of subpopulations -demes-;  Another model with resemblance with the well known cellular automata \cite{chopard1998cellular} was proposed several decades ago.  The \textit{cellular} model is thus a second possibility \cite{folino1999cellular}.  Similarly as with cellular automata, individuals are aligned on a grid, and each of them can only interact, by means of genetic operations, with their neighborhood. This way of interactions produces chromosome diffusion dynamics, that in the end, affects the evolutionary process \textit{tomassini2006spatially}.  

A number of researchers have relied in the model, successfully addressing hard problems.  Unfortunately, implementation details typically keeps this model to be widely-adopted by researchers:  differences with the standard sequential version of the algorithm are much larger now.

Comparing the three previously described parallel models, we see that when using the island model, each of the demes can run semi-isolated within each of the processors employed, and only a migrating step is required after a number of generations.  Nevertheless, the embarrassingly parallel model requires fitness values computed to be returned to the master in charge of applying each of the genetic operators, and this implies the sending of fitness values at least once per generation.  The ratio computation/communication may influence the performance of the algorithm: shorter time to compute fitness value means worse performance of the algorithm, given that the latency of communications has a larger impact. Similarly, this may also affect when using the cellular model, which requires communication among adjacent individuals from the topological point of view that are run on different processors every time a crossover operation must be applied. 

We can thus conclude that if distributed systems are employed to run some of the above described parallel models, latencies must be considered, which can deteriorate the speedup of both cellular and embarrassingly parallel model, even preventing them to compete in certain situations with the sequential version.  On the other hand, the island model will not be so severely affected by latencies, although of course, appropriate migrations frequencies must be chosen.

\subsection{Agent based models}

P2P models have allowed to implement new agent based EAs that
change the standard dynamics of the algorithm. Both models have changed the way
we understand the algorithm, and have shed light into some of the properties that the
new parallel models have unveiled \cite{DBLP:conf/eurogp/LaredoGVAG11}.

EXTEND THIS P2P MODELS HERE

Pool based models rely on a simple idea:  all the participants -computing nodes- of a distributed algorithm shares a single store of resources \cite{garcia2015evospace}.  In the case of EAs, the central store is in charge of maintaining the population of candidate solutions.  Although the model departs from the standard P2P, whose main feature is the lack of a central sever, still maintains the one of its main features:  all of the pairs behaves similarly, thus sharing responsabilities and tasks.

Therefore, a Pool-based EA notably differs from the more traditional \textit{embarrasingly parallel} model:  while in the latter the sever is in charge of every step but the fitness evaluation, in the pool-based model the sever only stores the individuals from the population, and are the peers which apply every genetic operation. Similarly, important differences may be noticed when compared with the \textit{island} model, given that every node in the island model communicates with the surronding islands during the migration steps, while in the case of the pool-based model, the communication is indirectly performed through the central population store.

==> parts_workshop/old/technologies.tex <==

 
 INFRASTRUCTURES - CLUSTER - GRID - DESKTOP GRIDS - CLOUD - P2P


When dealing with technologies required to deploy a parallel algorithm, which is born from the standard sequential version, two different kind of technologies must be considered:  (i) software libraries required for programming the parallel algorithm and (2) hardware required to run the new version of the algorithm.  We describe below some of the more commonly applied technologies, with some examples that have been developed in the last couple of decades, that allow us to see how both software and hardware have improved over the years.

\subsection{Hardware infrastructure}


\subsubsection{Grid and Desktop grids}

Although Grid technology was the promise in the new millennium to provide computing facilities everywhere, similarly as the electric grid provides power, the true is that the none of the standards, middleware and consortiums trying to establish the framework for grid computing were able to reach the goal \cite{grid}.  The main problem behind the \textit{grid idea} was heterogeneity:  very different computing resources connected, whit different hardware, operating systems, software libraries, etc.  Different middleware to chose from (glite, globus...);  different institutions trying to join the grid initiative with different internal policies.

Nevertheless, a much more modest approach only relying on desktop computers, was able to connect millions of users and computers providing a more standard and reliable distributed hardware infrastructure, gave rise to a different model:  \textit{Desktop grid}.

Desktop Grid Computing can be consider a particular case of Grid
technology where all of the computing resources are homogeneous: desktop personal
computers, with basically the same hardware architecture and a limited options for the operating system:  Linux, Windows or Os X;  which results on a  grid system that significantly simplifies
the way parallel algorithms can be deployed on the network of computers: a single
version of the algorithm must be implemented (linux?i386, for instance), instead of
considering all of the potential hardware architectures and operating systems combinations
that are present in a more traditional Grid infrastructure. 

%SEGUIR REESCRIBIENDO DESDE AQUÍ

Moreover, available
software tools, such as BOINC [13], allow to easily manage the desktop grid
infrastructure, allowing researchers to only focus on the Evolutionary Algorithm to
be deployed. The basic desktop-grid model follows the master-slave approach, and
is well suited to embarrassingly parallel EAs: typically desktop grids are deployed
within institutions, and communication latencies are thus under control.
The simplicity of desktop grids, has allowed researchers to face hard real life
problems: packages of individuals are distributed every generation along the available
computing nodes, allowing researchers to manage large population sizes for
real life problems requiring long fitness evaluation time [3]. Thus, the model was
shown to perfectly work on desktop grids provided by the researchers. The surprise
camewhen themodelwas applied using computing resources provided by volunteers
under the well known volunteer computing model [14].
Volunteer computing is based on the desktop grid model, and desktop computers
are provided by a number of volunteers connected to internet that are willing to
contribute to a scientific project. Thus, the scientist is typically in charge of setting
up the master node, where all of the computing tasks are established, and then, the
volunteers connect to the server and agree to provide computing resources for each
of the tasks. The model has worked fine for decades, being the Seti@home project
one of the best known with several million volunteers providing resources [13]. Nevertheless,
and given that resources are switched on and off according to volunteers?
needs, nobody can assure the time a computing node will be alive, and whether a specific
task submitted will be thus completed on time. The dynamic of the volunteer
computing infrastructure is thus characterize by this well known churn phenomena,
and scientists interested in profiting from volunteers must encode a number of faulttolerant
techniques if they want their project to finish properly [15]. But this inherent
property, churn, was recently considered from a different perspective in the context
of EAs, specifically from the point of view of Genetic Programming (GP) with
interesting results.


\subsection{Software libraries}

Regarding implementation details, communication libraries had to be selected when a parallel version of GP is to be implemented.  The first consideration for selecting the appropriate software tool or library is the kind of application to be parallelized, and the hardware infrastructure available.  According to Flynn taxonomy \cite{flynn2011flynn}, parallel GP can typically be considered a kind of SIMD application:  same operations (fitness evaluation in parallel for instance) applied to a set of data (candidate solutions within the population).   Although this kind of application could be run on any of the above described infrastructures, what we typically see in the literature, is the use of infrastructures that provide computing elements tight together.  Thus, grids are usually discarded because of communication latencies, and clusters are usually preferred.  Yet, in the last couple of years, new P2P models have been proposed that relies on cloud systems.

Traditionally PVM or MPI libraries \cite{geist1996pvm} has been employed when running parallel GP on clusters of computers.  Although PVM was the first choice back in the nineties, MPI has is a more mature technology that is nowadays available also in supercomputers.  Some standard GP software tools were adapted using these libraries in the past \cite{fernandez1999parallel}, \cite{tomassini2000mpi}.  Yet, in the last decade, some of the best known GP tools, such as ECJ, has incorporated parallel and distributed capabilities by using JAVA......

When considering grid computing, for instance, interesting software packages allow to quickly deploy any algorithm on an easy to build desktop grid system, such as that based in the BOINC framework [13], which has opened up a world of possibilities for parallel GP:  in the last decade an exhaustive study of the behavior of GP on this hardware infrastructure has allowed to show interesting properties that were not previously studied, such as \textit{fault-tolerance}.  Moreover, some of the best known software tools, such as ECJ, which includes the GP algorithm, has been adapted by researchers so that it can already be launched on BOINC based Desktop Grid system.  

Even the new \textit{map-reduce} model, that is available on \textit{Hadoop}, and allows to launch massive parallel computations on clusters, has also been used by researchers to launch parallel executions of EA experiments in connection with ECJ.

Finally, a P2P and agent based versions of the algorithms have been implemented in the EvoSpace model, which makes use of Redis, Cherrypy ........COMPLETE THIS




==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...´': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

